Excluding Single-Crossing Matching Minors in Bipartite Graphs

\noindent By a seminal result of Valiant, computing the permanent of $(0,1)$-matrices is, in general, $\#\mathsf{P}$-hard. In 1913 P\'olya asked for which $(0,1)$-matrices $A$ it is possible to change some signs such that the permanent of $A$ equals the determinant of the resulting matrix. In 1975, Little showed these matrices to be exactly the biadjacency matrices of bipartite graphs excluding $K_{3,3}$ as a \{matching minor}. This was turned into a polynomial time algorithm by McCuaig, Robertson, Seymour, and Thomas in 1999. However, the relation between the exclusion of some matching minor in a bipartite graph and the tractability of the permanent extends beyond $K_{3,3}.$ Recently it was shown that the exclusion of any planar bipartite graph as a matching minor yields a class of bipartite graphs on which the {permanent} of the corresponding $(0,1)$-matrices can be computed efficiently. In this paper we unify the two results above into a single, more general result in the style of the celebrated structure theorem for single-crossing-minor-free graphs. We identify a class of bipartite graphs strictly generalising planar bipartite graphs and $K_{3,3}$ which includes infinitely many non-Pfaffian graphs. The exclusion of any member of this class as a matching minor yields a structure that allows for the efficient evaluation of the permanent. Moreover, we show that the evaluation of the permanent remains $\#\mathsf{P}$-hard on bipartite graphs which exclude $K_{5,5}$ as a matching minor. This establishes a first computational lower bound for the problem of counting perfect matchings on matching minor closed classes.

==> figures/dp_ex_dp_hplo.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw[shift={(116.042, 780.175)}, xscale=0.5206, yscale=0.4876, darkmagenta, ipe pen heavier]
    (0, 0)
     -- (-40, 0)
     -- (-64, -32)
     -- (-24, -32)
     -- cycle;
  \draw[shift={(116.042, 780.175)}, xscale=0.5206, yscale=0.4876, darkmagenta]
    (0, 0)
     -- (-40, 0)
     -- (-64, -32)
     -- (-24, -32)
     -- cycle;
  \pic[ipe mark small]
     at (95.2166, 780.1746) {ipe disk};
  \pic[ipe mark small]
     at (103.5467, 764.5726) {ipe disk};
  \filldraw[shift={(95.217, 780.173)}, xscale=0.5206, yscale=0.4876, ipe pen ultrafat, fill=white]
    (0, 0)
     -- (0, 20);
  \draw[shift={(95.217, 789.924)}, xscale=0.5206, yscale=0.4876, darkred, ipe pen heavier]
    (0, 0)
     -- (0, -20);
  \pic[ipe mark small]
     at (95.2166, 780.1746) {ipe disk};


==> figures/k4opos.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw[darkmagenta]
    (188, 544)
     -- (148, 544)
     -- (124, 512)
     -- (164, 512)
     -- cycle;
  \pic
     at (148, 544) {ipe disk};
  \pic
     at (164, 512) {ipe disk};
  \filldraw[ipe pen ultrafat, fill=white]
    (148, 544)
     -- (148, 564);
  \draw[darkred, ipe pen heavier]
    (148, 564)
     -- (148, 544);
  \pic
     at (148, 544) {ipe disk};


==> figures/k4opos_copia.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \fill[lightblue, ipe opacity 75]
    (235.481, 409.8628)
     -- (239.47, 409.8578)
     -- (239.523, 399.9578)
     -- (255.523, 399.9578)
     -- (255.415, 410.1118)
     -- (259.449, 410.1528)
     -- (259.523, 395.9578)
     -- (235.523, 395.9578)
     -- (235.479, 409.8368);
  \fill[lightgreen, ipe opacity 75]
    (224.1352, 442.0327)
     -- (224.1352, 438.0327)
     -- (248.1352, 438.0327)
     -- (248.1352, 442.0327)
     -- (224.1352, 442.0327);
  \fill[lightblue, ipe opacity 75]
    (235.9253, 467.947)
     -- (239.9253, 467.947)
     -- (239.9253, 447.947)
     -- (255.9253, 447.947)
     -- (255.9253, 467.947)
     -- (259.9253, 467.947)
     -- (259.9253, 443.947)
     -- (235.9253, 443.947)
     -- (235.9253, 467.947);
  \fill[lightblue, ipe opacity 75]
    (171.953, 442.265)
     -- (175.953, 442.265)
     -- (175.953, 422.265)
     -- (191.953, 422.265)
     -- (191.953, 442.265)
     -- (195.953, 442.265)
     -- (195.953, 418.265)
     -- (171.953, 418.265)
     -- (171.953, 442.265);
  \fill[lightgreen, ipe opacity 75]
    (183.7926, 457.9908)
     -- (183.7926, 453.9908)
     -- (207.7926, 453.9908)
     -- (207.7926, 457.9908)
     -- (183.7926, 457.9908);
  \fill[lightgreen, ipe opacity 75]
    (48.1142, 399.984)
     -- (52.1142, 399.984)
     -- (52.0662, 385.842)
     -- (40.0662, 369.842)
     -- (36.0662, 369.842)
     -- (36.1142, 383.984)
     -- (40.1142, 383.984)
     -- (40.1262, 376.243)
     -- (48.1032, 387.403)
     -- (48.1142, 399.984);
  \fill[lightblue, ipe opacity 75]
    (27.948, 400.272)
     -- (31.948, 400.272)
     -- (31.9, 386.13)
     -- (19.9, 370.13)
     -- (15.9, 370.13)
     -- (15.948, 384.272)
     -- (19.948, 384.272)
     -- (19.96, 376.531)
     -- (27.937, 387.691)
     -- (27.948, 400.272);
  \fill[lightblue, ipe opacity 75]
    (80.0689, 400.212)
     -- (84.0689, 400.212)
     -- (84.0209, 386.07)
     -- (72.0209, 370.07)
     -- (68.0209, 370.07)
     -- (68.0689, 384.212)
     -- (72.0689, 384.212)
     -- (72.0809, 376.471)
     -- (80.0579, 387.631)
     -- (80.0689, 400.212);
  \fill[lightgreen, ipe opacity 75]
    (152.1705, 400.2397)
     -- (156.1705, 400.2397)
     -- (156.1705, 396.2397)
     -- (144.1705, 380.2397)
     -- (140.1705, 380.2397)
     -- (140.1705, 384.2397)
     -- (152.1705, 400.2397);
  \fill[lightblue, ipe opacity 75]
    (132.0781, 399.9743)
     -- (136.0781, 399.9743)
     -- (136.0781, 395.9743)
     -- (124.0781, 379.9743)
     -- (120.0781, 379.9743)
     -- (120.0781, 383.9743)
     -- (132.0781, 399.9743);
  \fill[lightgreen, ipe opacity 75]
    (100.0898, 399.802)
     -- (104.0898, 399.802)
     -- (104.0898, 395.802)
     -- (92.0898, 379.802)
     -- (88.0898, 379.802)
     -- (88.0898, 383.802)
     -- (100.0898, 399.802);
  \fill[lightgreen, ipe opacity 75]
    (152.1036, 458.4318)
     -- (156.1036, 458.4318)
     -- (156.1036, 454.4318)
     -- (144.1036, 438.4318)
     -- (140.1036, 438.4318)
     -- (140.1036, 442.4318)
     -- (152.1036, 458.4318);
  \fill[lightblue, ipe opacity 75]
    (132.0112, 458.1664)
     -- (136.0112, 458.1664)
     -- (136.0112, 454.1664)
     -- (124.0112, 438.1664)
     -- (120.0112, 438.1664)
     -- (120.0112, 442.1664)
     -- (132.0112, 458.1664);
  \fill[lightgreen, ipe opacity 75]
    (100.0229, 457.9941)
     -- (104.0229, 457.9941)
     -- (104.0229, 453.9941)
     -- (92.0229, 437.9941)
     -- (88.0229, 437.9941)
     -- (88.0229, 441.9941)
     -- (100.0229, 457.9941);
  \fill[lightblue, ipe opacity 75]
    (79.9638, 457.99)
     -- (83.9638, 457.99)
     -- (84, 416)
     -- (68, 416)
     -- (67.9638, 441.99)
     -- (71.9638, 441.99)
     -- (72, 420)
     -- (80, 420)
     -- (79.9638, 457.99);
  \fill[lightgreen, ipe opacity 75]
    (47.9638, 457.99)
     -- (51.9638, 457.99)
     -- (52, 416)
     -- (36, 416)
     -- (35.9638, 441.99)
     -- (39.9638, 441.99)
     -- (40, 420)
     -- (48, 420)
     -- (47.9638, 457.99);
  \fill[lightblue, ipe opacity 75]
    (27.9638, 457.99)
     -- (31.9638, 457.99)
     -- (32, 416)
     -- (16, 416)
     -- (15.9638, 441.99)
     -- (19.9638, 441.99)
     -- (20, 420)
     -- (28, 420)
     -- (27.9638, 457.99);
  \fill[lightblue, ipe opacity 75]
    (184.052, 513.996)
     -- (187.995, 514.023)
     -- (188, 504)
     -- (204, 504)
     -- (204.041, 514.114)
     -- (208.012, 514.089)
     -- (208, 500)
     -- (184, 500)
     -- (184.062, 513.951);
  \fill[lightgreen, ipe opacity 75]
    (172, 488)
     -- (172, 484)
     -- (196, 484)
     -- (196, 488)
     -- (172, 488);
  \fill[lightblue, ipe opacity 75]
    (256, 572)
     -- (260, 572)
     -- (260.033, 522.262)
     -- (244.033, 522.262)
     -- (244.033, 546.262)
     -- (248.033, 546.262)
     -- (248.033, 526.262)
     -- (256.033, 526.262)
     -- (256.033, 570.262);
  \fill[lightgreen, ipe opacity 75]
    (236, 572)
     -- (240, 572)
     -- (240.033, 522.262)
     -- (224.033, 522.262)
     -- (224.033, 546.262)
     -- (228.033, 546.262)
     -- (228.033, 526.262)
     -- (236.033, 526.262)
     -- (236.033, 570.262);
  \fill[lightgreen, ipe opacity 75]
    (172.0332, 546.0415)
     -- (176.0332, 546.0415)
     -- (176.0332, 526.0415)
     -- (192.0332, 526.0415)
     -- (192.0332, 546.0415)
     -- (196.0332, 546.0415)
     -- (196.0332, 522.0415)
     -- (172.0332, 522.0415)
     -- (172.0332, 546.0415);
  \fill[lightblue, ipe opacity 75]
    (184, 572)
     -- (188, 572)
     -- (188, 552)
     -- (204, 552)
     -- (204, 572)
     -- (208, 572)
     -- (208, 548)
     -- (184, 548)
     -- (184, 572);
  \fill[lightgreen, ipe opacity 75]
    (28, 572)
     -- (32, 572)
     -- (32, 532)
     -- (36, 532)
     -- (36, 556)
     -- (40, 556)
     -- (40, 528)
     -- (28, 528)
     -- (28, 572);
  \fill[lightblue, ipe opacity 75]
    (152, 572)
     -- (156, 572)
     -- (156, 520)
     -- (120, 520)
     -- (120.018, 546.312)
     -- (124.023, 546.317)
     -- (124, 524)
     -- (152, 524)
     -- (152, 572);
  \fill[lightgreen, ipe opacity 75]
    (132, 572)
     -- (136, 572)
     -- (136, 532)
     -- (140, 532)
     -- (140.013, 546.131)
     -- (144.02, 546.147)
     -- (144, 528)
     -- (132, 528)
     -- (132, 572);
  \fill[lightgreen, ipe opacity 75]
    (100.048, 514.142)
     -- (104.048, 514.142)
     -- (104, 500)
     -- (92, 484)
     -- (88, 484)
     -- (88.048, 498.142)
     -- (92.048, 498.142)
     -- (92.06, 490.401)
     -- (100.037, 501.561)
     -- (100.048, 514.142);
  \fill[lightgreen, ipe opacity 75]
    (100, 572)
     -- (104, 572)
     -- (104, 528)
     -- (88, 528)
     -- (88, 556)
     -- (92, 556)
     -- (92, 532)
     -- (100, 532)
     -- (100, 572);
  \fill[lightblue, ipe opacity 75]
    (80.048, 514.142)
     -- (84.048, 514.142)
     -- (84, 500)
     -- (72, 484)
     -- (68, 484)
     -- (68.048, 498.142)
     -- (72.048, 498.142)
     -- (72.06, 490.401)
     -- (80.037, 501.561)
     -- (80.048, 514.142);
  \fill[lightblue, ipe opacity 75]
    (80, 572)
     -- (84, 572)
     -- (84, 528)
     -- (68, 528)
     -- (68, 556)
     -- (72, 556)
     -- (72, 532)
     -- (80, 532)
     -- (80, 572);
  \draw[shift={(102, 560)}, scale=0.5, darkmagenta]
    (0, 0)
     -- (-40, 0)
     -- (-64, -32)
     -- (-24, -32)
     -- cycle;
  \pic
     at (82, 560) {ipe disk};
  \pic
     at (90, 544) {ipe disk};
  \filldraw[shift={(82, 560)}, scale=0.5, ipe pen ultrafat, fill=white]
    (0, 0)
     -- (0, 20);
  \draw[shift={(82, 570)}, scale=0.5, darkred, ipe pen heavier]
    (0, 0)
     -- (0, -20);
  \pic
     at (82, 560) {ipe disk};


==> figures/separtors_dibraces.tex <==
\tikzstyle{ipe stylesheet} = [
  ipe import,
  even odd rule,
  line join=round,
  line cap=butt,
  ipe pen normal/.style={line width=0.4},
  ipe pen heavier/.style={line width=0.8},
  ipe pen fat/.style={line width=1.2},
  ipe pen ultrafat/.style={line width=2},
  ipe pen normal,
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark normal,
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=7},
  ipe arrow large/.style={scale=10},
  ipe arrow small/.style={scale=5},
  ipe arrow tiny/.style={scale=3},
  ipe arrow normal,
  /tikz/.cd,
  ipe arrows, % update arrows
  <->/.tip = ipe normal,
  ipe dash normal/.style={dash pattern=},
  ipe dash dotted/.style={dash pattern=on 1bp off 3bp},
  ipe dash dashed/.style={dash pattern=on 4bp off 4bp},
  ipe dash dash dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp},
  ipe dash dash dot dotted/.style={dash pattern=on 4bp off 2bp on 1bp off 2bp on 1bp off 2bp},
  ipe dash normal,
  ipe node/.append style={font=\normalsize},
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe opacity 10/.style={opacity=0.1},
  ipe opacity 30/.style={opacity=0.3},
  ipe opacity 50/.style={opacity=0.5},
  ipe opacity 75/.style={opacity=0.75},
  ipe opacity opaque/.style={opacity=1},
  ipe opacity opaque,
]
\definecolor{red}{rgb}{1,0,0}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{green}{rgb}{0,1,0}
\definecolor{yellow}{rgb}{1,1,0}
\definecolor{orange}{rgb}{1,0.647,0}
\definecolor{gold}{rgb}{1,0.843,0}
\definecolor{purple}{rgb}{0.627,0.125,0.941}
\definecolor{gray}{rgb}{0.745,0.745,0.745}
\definecolor{brown}{rgb}{0.647,0.165,0.165}
\definecolor{navy}{rgb}{0,0,0.502}
\definecolor{pink}{rgb}{1,0.753,0.796}
\definecolor{seagreen}{rgb}{0.18,0.545,0.341}
\definecolor{turquoise}{rgb}{0.251,0.878,0.816}
\definecolor{violet}{rgb}{0.933,0.51,0.933}
\definecolor{darkblue}{rgb}{0,0,0.545}
\definecolor{darkcyan}{rgb}{0,0.545,0.545}
\definecolor{darkgray}{rgb}{0.663,0.663,0.663}
\definecolor{darkgreen}{rgb}{0,0.392,0}
\definecolor{darkmagenta}{rgb}{0.545,0,0.545}
\definecolor{darkorange}{rgb}{1,0.549,0}
\definecolor{darkred}{rgb}{0.545,0,0}
\definecolor{lightblue}{rgb}{0.678,0.847,0.902}
\definecolor{lightcyan}{rgb}{0.878,1,1}
\definecolor{lightgray}{rgb}{0.827,0.827,0.827}
\definecolor{lightgreen}{rgb}{0.565,0.933,0.565}
\definecolor{lightyellow}{rgb}{1,1,0.878}
\definecolor{black}{rgb}{0,0,0}
\definecolor{white}{rgb}{1,1,1}
\begin{tikzpicture}[ipe stylesheet]
  \draw[darkorange]
    (276.054, 712.256)
     .. controls (260.018, 704.0853) and (251.917, 693.4953) .. (251.751, 680.486);
  \draw[seagreen, ipe pen ultrafat, -{ipe arc[ipe arrow small]}]
    (252, 680)
     -- (252, 700);


==> tikzlibraryipe.code.tex <==

% Copyright (C) 2016  Joseph Rabinoff

% ipe2tikz is free software; you can redistribute it and/or modify it under
% the terms of the GNU General Public License as published by the Free
% Software Foundation; either version 3 of the License, or (at your option)
% any later version.

% ipe2tikz is distributed in the hope that it will be useful, but WITHOUT ANY
% WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the GNU General Public License for more
% details.

% You should have received a copy of the GNU General Public License along with
% ipe2tikz; if not, you can find it at "http://www.gnu.org/copyleft/gpl.html",
% or write to the Free Software Foundation, Inc., 675 Mass Ave, Cambridge, MA
% 02139, USA.


% ipe compatibility TikZ styles

\usetikzlibrary{arrows.meta}

\makeatletter

% These should behave almost exactly like ipe arrows.  They disable correcting
% for the miter length and line width.  This is important for visual consistency
% with ipe, since ipe arrows get much larger when the line width is increased.
% They also use the line join and cap styles from the main path.  These are very
% simple arrows: there is no harpoon version, and the convex hull computation is
% sloppy.

\pgfdeclarearrow{
  name = ipe _linear,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{
      \pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \pgfarrowssetlineend{\pgfarrowlength}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength\advance\pgf@x by-.5\pgfarrowlinewidth}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfusepathqstroke
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
  },
}


\pgfdeclarearrow{
  name = ipe _pointed,
  defaults = {
    length = +1bp,
    width  = +.666bp,
    inset  = +.2bp,
    line width = +0pt 1,
  },
  setup code = {
    % Control points
    \pgfarrowssetbackend{0pt}
    \pgfarrowssetvisualbackend{\pgfarrowinset}
    \pgfarrowssetlineend{\pgfarrowinset}
    \ifpgfarrowreversed
      \pgfarrowssetlineend{\pgfarrowlength}
    \fi
    \pgfarrowssettipend{\pgfarrowlength}
    % Convex hull
    \pgfarrowshullpoint{\pgfarrowlength}{0pt}
    \pgfarrowsupperhullpoint{0pt}{.5\pgfarrowwidth}
    \pgfarrowshullpoint{\pgfarrowinset}{0pt}
    % The following are needed in the code:
    \pgfarrowssavethe\pgfarrowinset
    \pgfarrowssavethe\pgfarrowlinewidth
    \pgfarrowssavethe\pgfarrowlength
    \pgfarrowssavethe\pgfarrowwidth
  },
  drawing code = {
    \pgfsetdash{}{+0pt}
    \ifdim\pgfarrowlinewidth=\pgflinewidth\else\pgfsetlinewidth{+\pgfarrowlinewidth}\fi
    \pgfpathmoveto{\pgfqpoint{\pgfarrowlength}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{.5\pgfarrowwidth}}
    \pgfpathlineto{\pgfqpoint{\pgfarrowinset}{0pt}}
    \pgfpathlineto{\pgfqpoint{0pt}{-.5\pgfarrowwidth}}
    \pgfpathclose
    \ifpgfarrowopen
      \pgfusepathqstroke
    \else
      \ifdim\pgfarrowlinewidth>0pt\pgfusepathqfillstroke\else\pgfusepathqfill\fi
    \fi
  },
  parameters = {
    \the\pgfarrowlinewidth,%
    \the\pgfarrowlength,%
    \the\pgfarrowwidth,%
    \the\pgfarrowinset,%
    \ifpgfarrowopen o\fi%
  },
}


% For correcting minipage width in stretched nodes
\newdimen\ipeminipagewidth
\def\ipestretchwidth#1{%
  \pgfmathsetlength{\ipeminipagewidth}{#1/\ipenodestretch}}

\tikzstyle{ipe import} = [
  % General ipe defaults
  x=1bp, y=1bp,
%
  % Nodes
  ipe node stretch/.store in=\ipenodestretch,
  ipe stretch normal/.style={ipe node stretch=1},
  ipe stretch normal,
  ipe node/.style={
    anchor=base west, inner sep=0, outer sep=0, scale=\ipenodestretch
  },
%
  % Use a special key for the mark scale, so that the default can be overriden.
  % (This doesn't happen with the scale= key; those accumulate.)
  ipe mark scale/.store in=\ipemarkscale,
%
  ipe mark tiny/.style={ipe mark scale=1.1},
  ipe mark small/.style={ipe mark scale=2},
  ipe mark normal/.style={ipe mark scale=3},
  ipe mark large/.style={ipe mark scale=5},
%
  ipe mark normal, % Set default
%
  ipe circle/.pic={
    \draw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe disk/.pic={
    \fill (0,0) circle[radius=0.6*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe fdisk/.pic={
    \filldraw[line width=0.2*\ipemarkscale]
      (0,0) circle[radius=0.5*\ipemarkscale];
    \coordinate () at (0,0);
  },
  ipe box/.pic={
    \draw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe square/.pic={
    \fill
      (-.6*\ipemarkscale,-.6*\ipemarkscale) rectangle
      ( .6*\ipemarkscale, .6*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe fsquare/.pic={
    \filldraw[line width=0.2*\ipemarkscale, line join=miter]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) rectangle
      ( .5*\ipemarkscale, .5*\ipemarkscale);
    \coordinate () at (0,0);
  },
  ipe cross/.pic={
    \draw[line width=0.2*\ipemarkscale, line cap=butt]
      (-.5*\ipemarkscale,-.5*\ipemarkscale) --
      ( .5*\ipemarkscale, .5*\ipemarkscale)
      (-.5*\ipemarkscale, .5*\ipemarkscale) --
      ( .5*\ipemarkscale,-.5*\ipemarkscale);
    \coordinate () at (0,0);
  },
%
  % Arrow sizes (for TikZ arrows)
  /pgf/arrow keys/.cd,
  ipe arrow normal/.style={scale=1},
  ipe arrow tiny/.style={scale=.4},
  ipe arrow small/.style={scale=.7},
  ipe arrow large/.style={scale=1.4},
  ipe arrow normal,
  /tikz/.cd,
%
  % Approximations to ipe arrows
  % Put in a style to allow to reset default scale when "ipe arrow normal" is
  % changed.  I think this is the only way, since all the parameters to arrows
  % are expanded when the tip is declared.
  ipe arrows/.style={
    ipe normal/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0bp,
                   quick, ipe arrow normal]},
    ipe pointed/.tip={
      ipe _pointed[length=1bp, width=.666bp, inset=0.2bp,
                   quick, ipe arrow normal]},
    ipe linear/.tip={
      ipe _linear[length = 1bp, width=.666bp,
                  ipe arrow normal, quick]},
    ipe fnormal/.tip={ipe normal[fill=white]},
    ipe fpointed/.tip={ipe pointed[fill=white]},
    ipe double/.tip={ipe normal[] ipe normal},
    ipe fdouble/.tip={ipe fnormal[] ipe fnormal},
    % These should maybe use [bend], but that often looks bad unless it's on an
    % actual arc.
    ipe arc/.tip={ipe normal},
    ipe farc/.tip={ipe fnormal},
    ipe ptarc/.tip={ipe pointed},
    ipe fptarc/.tip={ipe fpointed},
  },
  ipe arrows, % Set default sizes
]

% I'm not sure how to do this in a .style, since the #args get confused.
\tikzset{
  rgb color/.code args={#1=#2}{%
    \definecolor{tempcolor-#1}{rgb}{#2}%
    \tikzset{#1=tempcolor-#1}%
  },
}

\makeatother

\endinput

